Efficient Measurement of Complex Networks Using Link Queries

Complex networks are at the core of an intense research activity. However, in most cases, intricate and costly measurement procedures are needed to explore their structure. In some cases, these measurements rely on link queries: given two nodes, it is possible to test the existence of a link between them. These tests may be costly, and thus minimizing their number while maximizing the number of discovered links is a key issue. This paper studies this problem: we observe that properties classically observed on real-world complex networks give hints for their efficient measurement; we derive simple principles and several measurement strategies based on this, and experimentally evaluate their efficiency on real-world cases. In order to do so, we introduce methods to evaluate the efficiency of strategies. We also explore the bias that different measurement strategies may induce.

==> algo.tex <==
\begin{algorithm}[H]
\caption{\tracetree\ algorithm.}
\SetCommentSty{small}
\dontprintsemicolon
\SetKw{Or}{or}
\SetKw{KwIf}{if}
%\SetKw{And}{and}
\SetKw{Output}{print}
\SetKw{Gets}{$\leftarrow$\ }
\KwIn{set $D$ of destinations, with $d\in D$ at distance $ttl_d$.}
$to\_probe$ \Gets empty queue,
$to\_receive$ \Gets $\emptyset$,
$seen$ \Gets $\emptyset$\;
\lForEach{$d \in D$}{add $(d,ttl_d)$ to $to\_probe$}\;
\While{$to\_probe$ not empty \Or $to\_receive \not= \emptyset$}{
 \lnlset{send_strategy}{$\alpha$}%
 \If{$to\_probe$ not empty}{
  pop $(d,ttl)$ from $to\_probe$ and send a probe to it\;
  add $(d,ttl,current\_time())$ to $to\_receive$\;
  }
 \tcp{here necessarily $to\_receive \not= \emptyset$}
% $p$ \Gets read {\sc icmp} packet\hfill\tcp{non-blocking}
 \lnlset{check_packet}{$\beta$}%
 \If{answer $p$ to a probe to $(d,ttl)$ received}{
  \tcp{$p$ sent by $p.source$, reply to a probe to $(d,ttl)$}
%  \If(\hfill\CommentSty{// else timeout}){$(d,ttl,\_) \in to\_receive$}{
  \If{$(d,ttl,\_) \in to\_receive$}{
    \tcp{else timeout}
    remove $(d,ttl,\_)$ from $to\_receive$;\\
   \Output $p.source$ $ttl$ $d$\;
   \If{$(p.source,ttl) \not\in seen$}{
    add $(p.source,ttl)$ to $seen$\;
    push $(d,ttl-1)$ in $to\_probe$ \KwIf $ttl>1$\;
    }
   }
  }
 \For{$(d,ttl,t) \in to\_receive$ \KwIf timeout exceeded}{
   remove $(d,ttl,t)$ from $to\_receive$\;
   \Output * $ttl$ $d$\;
   \If{$ttl>1$}{
   push $(d,ttl-1)$ in $to\_probe$\;
 }
  }
 }
\label{algo_tracetree}
\end{algorithm}


